Canonical quotients in model theory

We study canonical quotients in model theory, mainly stable quotients of type-definable groups and invariant types in NIP theories. We extend the modelling property to continuous theories and use it to study $n$-dependence in hyperdefinable sets. Furthermore, we study maximal WAP and tame quotients of $S_X(\mathfrak{C})$, where $\mathfrak{C}$ is a monster model of a complete theory $T$ and $X$ is an $\emptyset$-type-definable set and show that the Ellis groups of the maximal WAP quotient flow and the maximal tame quotient flow do not depend on the choice of the monster model $\mathfrak{C}$.

==> abstract_polish.tex <==
\fancyhf{} % clear all header and footer fields
\fancyhead[RO,R]{\thepage} %RO=right odd, RE=right even
\renewcommand{\headrulewidth}{0pt}

\begin{center}
    %\Large
    %\textbf{Thesis Title}
    
    %\vspace{0.4cm}
    %\large
    %Thesis Subtitle
    
    %%\vspace{0.4cm}
    %\textbf{Author Name}
    
   % \vspace{0.9cm}
    \textbf{Streszczenie}
\end{center}

Badamy ilorazy kanoniczne w teorii modeli, g\l ównie stabilne ilorazy grup definiowalnych przez typ oraz typy niezmienników w teoriach NIP.

G\l ówne wyniki rozprawy s\c a nast\c epuj\c ace:
\begin{itemize}
    \item Rozwi\c azujemy dwa problemy dotycz\c ace maksymalnych stabilnych ilorazów grup definiowalnych przez typ w teoriach NIP. Pierwszy wynik mówi, \.ze je\'sli $G$ jest grup\c a definiowaln\c a w teorii dystalnej, to $G^{st}=G^{00}$ (gdzie $G^{st}$ jest najmniejsz\c a podgrup\c a definiowaln\c a ze stabilnym $G/G^{st}$, a $G^{00}$ jest najmniejsz\c a podgrup\c a definiowaln\c a o ograniczonym indeksie). Aby go uzyska\'c, dowodzimy, \.ze dystalno\'s\'c jest zachowana przy przej\'sciu od $T$ do hiperurojonego rozwini\c ecia???(verify) $T^{heq}$. Drugim wynikiem jest przyk\l ad grupy $G$ definiowalnej w niedystalnej teorii NIP, dla której $G=G^{00}$, ale $G^{st}$ nie jest przeci\c eciem grup definiowalnych. Naszym przyk\l adem jest nasycone rozszerzenie $(\mathbb{R},+,[0,1])$. Ponadto poczynili\'smy pewne obserwacje dotycz\c ace pytania, czy istnieje taki przyk\l ad, który jest grup\c a o skończonym wyk\l adniku. Korzystaj\c ac z okazji podajemy kilka charakterystyk stabilno\'sci zbiorów hiperdefiniowalnych, obejmuj\c acych logik\c e ci\c ag\l \c a.

    \item Dla teorii NIP $T$, dostatecznie nasyconego modelu $\C$ teorii $T$ (tzw. modelu monstrum) oraz niezmienniczego (na pewnym ma\l ym podzbiorze $\C$) globalnego typu $p$ dowodzimy, \.ze istnieje najmniejsza relatywnie definiowalna przez typ relacja równowa\.zno\'sci na ma\l ym zbiorze parametrów z $\C$ na zbiorze realizacji $p$, która ma stabilny iloraz. Jest to odpowiednik relacji równowa\.zno\'sci g\l ównego wyniku \cite{MR3796277} na istnienie maksymalnych stabilnych ilorazów grup definiowalnych przez typ w teoriach NIP. Nasz dowód adaptuje idee dowodu tego wyniku, dzia\l aj\c ac na wzgl\c ednie definiowalnych typowo podzbiorach grupy automorfizmów modelu monstrum zdefiniowanego w \cite{hrushovski2021order}.

    \item Definiujemy w\l a\'sciwo\'s\'c ci\c ag\l ego modelowania dla struktur pierwszego rz\c edu i pokazujemy, \.ze struktura pierwszego rz\c edu ma w\l a\'sciwo\'s\'c ci\c ag\l ego modelowania wtedy i tylko wtedy, gdy jej wiek ma w\l a\'sciwo\'s\'c osadzania Ramseya. U\.zywamy uogólnionych nierozró\.znialnych sekwencji w logice ci\c ag\l ej do badania i charakteryzowania zale\.zno\'sci $n$ dla teorii ci\c ag\l ych i hiperdefiniowalnych zbiorów pierwszego rz\c edu w kategoriach upadku nierozró\.znialnych sekwencji.
    \item Badamy maksymalne WAP i ograniczone??????tame (verify) (w sensie dynamiki topologicznej) ilorazy $S_X(\C)$, gdzie $\C$ jest modelem monstrum teorii pe\l nej $T$, a $X$ jest zbiorem definiowalnym typu $\emptyset$. Mianowicie, niech $\fwap\subset S_X(\C)\times S_X(\C)$ b\c edzie najmniejsz\c a domkni\c et\c a niezmiennicz\c a relacj\c a równowa\.zno\'sci $\aut(\C)$ na $S_X(\C)$ tak\c a, \.ze przep\l yw $( \aut(\C), S_X(\C)/\fwap)$ jest WAP, i niech $\fta\subset S_X(\C)\times S_X(\C)$ b\c edzie najmniejsz\c a domkni\c et\c a niezmiennicz\c a relacj\c a równowa\.zno\'sci $\aut(\C)$ na $S_X(\C)$ tak\c a, \.ze przep\l yw $( \aut(\C), S_X(\C)/\fta )$ jest ograniczone??? (verify). Wykazujemy dobre zachowanie $\fwap$ i $\fta$ przy zmianie modelu monstrum $\C$. Mianowicie, dowodzimy, \.ze je\'sli $\C'\succ \C$ jest wi\c ekszym modelem monstrum, to $\fwapp$ i $\ftaa$ s\c a odpowiednikami $\fwap$ i $\fta$ obliczonymi dla $\C'$ i $r: S_X(\C')\to S_X(\C)$ jest map ograniczaj\c ac\c a, to $r[\fwapp]=\fwap$ i $r[\ftaa]=\fta$. Korzystaj\c ac z tych wyników, pokazujemy, \.ze grupy Ellisa $( \aut(\C), S_X(\C)/\fwap )$ i $( \aut(\C), S_X(\C)/\fta )$ nie zale\.z\c a od wyboru modelu monstrum $\C$.
\end{itemize}

Wyniki zawarte w pierwszym, drugim i czwartym punkcie s\c a wynikami badań przeprowadzonych wspólnie z Krzysztofem Krupińskim, a te zawarte w trzecim punkcie s\c a moje w\l asne.

